Large Language Models for Automated Data Science: Introducing CAAFE for Context-Aware Automated Feature Engineering

As the field of automated machine learning (AutoML) advances, it becomes increasingly important to incorporate domain knowledge into these systems. We present an approach for doing so by harnessing the power of large language models (LLMs). Specifically, we introduce Context-Aware Automated Feature Engineering (CAAFE), a feature engineering method for tabular datasets that utilizes an LLM to iteratively generate additional semantically meaningful features for tabular datasets based on the description of the dataset. The method produces both Python code for creating new features and explanations for the utility of the generated features. Despite being methodologically simple, CAAFE improves performance on 11 out of 14 datasets -- boosting mean ROC AUC performance from 0.798 to 0.822 across all dataset - similar to the improvement achieved by using a random forest instead of logistic regression on our datasets. Furthermore, CAAFE is interpretable by providing a textual explanation for each generated feature. CAAFE paves the way for more extensive semi-automation in data science tasks and emphasizes the significance of context-aware solutions that can extend the scope of AutoML systems to semantic AutoML. We release our $\href{https://github.com/automl/CAAFE}{code}$, a simple $\href{https://colab.research.google.com/drive/1mCA8xOAJZ4MaB_alZvyARTMjhl6RZf0a}{demo}$ and a $\href{https://pypi.org/project/caafe/}{python\ package}$.

==> figures/full_results.tex <==
% \\textbf{} ([0-9\.]*)  ->  \textbf{$1} 
% Replace $\langle Kaggle\rangle$ with $\langle Kaggle\rangle$
\footnotesize
\begin{tabular}{l|r|rrrr|rrrr}
\toprule
{} & \multicolumn{1}{c}{Log. Reg.} & \multicolumn{4}{c}{Random Forest} & \multicolumn{4}{c}{TabPFN} \\
Dataset & \textbf{$\emptyset$} & \textbf{$\emptyset$} &  \textbf{AF} &  \textbf{DFS} & \textbf{\methodname{}}  & \textbf{$\emptyset$}  &  \textbf{AE} &  \textbf{DFS} & \textbf{\methodname{}} \\
\midrule
airlines & 0.620 & 0.635 & \textbf{0.662}  & 0.653 & 0.633 & 0.621 & \textbf{0.645}  & 0.634 & 0.620 \\
balance-scale & 0.773 & 0.695 & 0.704 & 0.750 & \textbf{0.831}  & 0.844 & 0.849 & 0.845 & \textbf{0.882}  \\
breast-w & 0.983 & 0.981 & 0.973 & \textbf{0.986}  & 0.985 & 0.978 & 0.971 & 0.978 & \textbf{0.981}  \\
cmc & 0.690 & 0.693 & 0.689 & \textbf{0.699}  & 0.692 & 0.737 & 0.737 & 0.735 & \textbf{0.739}  \\
credit-g & 0.767 & 0.775 & \textbf{0.782}  & 0.769 & 0.777 & 0.782 & \textbf{0.783}  & 0.782 & \textbf{0.783}  \\
diabetes & 0.836 & 0.825 & 0.822 & \textbf{0.827}  & 0.824 & \textbf{0.843}  & 0.841 & 0.841 & \textbf{0.843}  \\
eucalyptus & 0.881 & 0.910 & \textbf{0.920}  & 0.916 & 0.908 & \textbf{0.932}  & \textbf{0.932}  & \textbf{0.932}  & \textbf{0.932}  \\
jungle\_chess.. & 0.784 & 0.923 & 0.913 & 0.924 & \textbf{0.935}  & 0.933 & 0.922 & 0.924 & \textbf{0.945}  \\
$\langle KG\rangle$ health-insurance & 0.565 & \textbf{0.567}  & 0.562 & 0.522 & 0.556 & 0.574 & 0.574 & 0.537 & \textbf{0.575}  \\
$\langle KG\rangle$ pharyngitis & 0.680 & 0.687 & 0.686 & 0.693 & \textbf{0.699}  & 0.698 & 0.686 & 0.687 & \textbf{0.708}  \\
$\langle KG\rangle$ kidney-stone & 0.773 & 0.771 & 0.787 & \textbf{0.791}  & 0.785 & 0.788 & \textbf{0.793}  & 0.792 & 0.790 \\
$\langle KG\rangle$ spaceship-titanic & 0.828 & 0.813 & \textbf{0.832}  & 0.812 & 0.815 & 0.838 & \textbf{0.844}  & 0.841 & 0.840 \\
pc1 & 0.775 & 0.852 & 0.870 & \textbf{0.874}  & 0.860 & 0.903 & 0.908 & 0.908 & \textbf{0.909}  \\
tic-tac-toe & 0.601 & 0.821 & 0.806 & 0.769 & \textbf{0.951}  & 0.699 & 0.693 & 0.633 & \textbf{0.954}  \\
\midrule
Mean ROC & 0.754 & 0.782 & 0.786 & 0.785 & \textbf{0.804}  & 0.798 & 0.798 & 0.791 & \textbf{0.822}  \\
\bottomrule
\end{tabular}

==> figures/results_CAFE_only.tex <==
\footnotesize
\begin{tabular}{l|r|r|rr}
\toprule
{} & \multicolumn{1}{c}{Log. Reg.} & \multicolumn{1}{c}{Random Forest} & \multicolumn{2}{c}{TabPFN} \\
Dataset &  &  &  \textbf{$\emptyset$}  & \textbf{\methodname{}} \\
\midrule
airlines & 0.620 & 0.635 & \textbf{0.621} & 0.620 \\
balance-scale & 0.773 & 0.695 & 0.844 & \textbf{0.882} \\
breast-w & 0.983 & 0.981 & 0.978 & \textbf{0.981} \\
cmc & 0.690 & 0.693 & 0.737 & \textbf{0.739} \\
credit-g & 0.767 & 0.775 & 0.782 & \textbf{0.783} \\
diabetes & 0.836 & 0.825 & \textbf{0.843} & \textbf{0.843} \\
eucalyptus & 0.881 & 0.910 & \textbf{0.932} & \textbf{0.932} \\
jungle\_chess.. & 0.784 & 0.923 & 0.933 & \textbf{0.945} \\
$\langle Kaggle\rangle$ health-insurance & 0.565 & 0.567 & 0.574 & \textbf{0.575} \\
$\langle Kaggle\rangle$ pharyngitis & 0.680 & 0.687 & 0.698 & \textbf{0.708} \\
$\langle Kaggle\rangle$ kidney-stone & 0.773 & 0.771 & 0.788 & \textbf{0.790} \\
$\langle Kaggle\rangle$ spaceship-titanic & 0.828 & 0.813 & 0.838 & \textbf{0.840} \\
pc1 & 0.775 & 0.852 & 0.903 & \textbf{0.909} \\
tic-tac-toe & 0.601 & 0.821 & 0.699 & \textbf{0.954} \\
\midrule
Mean ROC & 0.754 & 0.782 & 0.798 & \textbf{0.822} \\
\end{tabular}

==> figures/results_cafe_and_baselines.tex <==
\begin{table}[H]
    \label{table:proposal}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{5pt}
\begin{tabular}{lll|ll|ll|ll}
\toprule
{} & {} & \multicolumn{1}{c}{No FE} & \multicolumn{2}{c}{AutoFE-Base} & \multicolumn{2}{c}{CAAFE} & \multicolumn{2}{c}{AutoFE-Base + CAAFE} \\
{} & &  & AutoFeat & DFS & GPT-3.5 & GPT-4 & GPT-4 + AF & GPT-4 + DFS \\
\midrule
Log. Reg.      & Mean &  0.749 {\tiny $\pm$.14} &  0.754 {\tiny $\pm$.14} &  0.764 {\tiny $\pm$.14} &   0.75 {\tiny $\pm$.14} &           0.769 {\tiny $\pm$.13} &           0.781 {\tiny $\pm$.14} &  \textbf{0.784} {\tiny $\pm$.14} \\
\rowcolor{gray!25}
      & Mean Rank &  5.11 &     4.21 &  3.36 &  4.79 &           4.31 &           3.52 &  \textbf{2.69} \\
\midrule
Rand. Forest & Mean &  0.783 {\tiny $\pm$.13} &  0.782 {\tiny $\pm$.12} &  0.781 {\tiny $\pm$.14} &  0.783 {\tiny $\pm$.13} &           0.801 {\tiny $\pm$.14} &  \textbf{0.808} {\tiny $\pm$.14} &           0.808 {\tiny $\pm$.14} \\
\rowcolor{gray!25}
 & Mean Rank &  4.44 &     4.41 &  4.14 &  4.38 &           4.28 &  \textbf{3.15} &           3.21 \\
\midrule
TabPFN   & Mean &  0.798 {\tiny $\pm$.14} &  0.797 {\tiny $\pm$.14} &  0.791 {\tiny $\pm$.15} &  0.799 {\tiny $\pm$.14} &  \textbf{0.822} {\tiny $\pm$.14} &           0.821 {\tiny $\pm$.14} &           0.818 {\tiny $\pm$.14} \\
\rowcolor{gray!25}
   & Mean Rank &  4.39 &      4.4 &  4.76 &  4.26 &  \textbf{3.06} &           3.27 &           3.86 \\
\bottomrule
\end{tabular}
\end{table}

==> figures/results_per_ds_plus_baselines_limited.tex <==
\begin{tabular}{ll|ll|ll}
\toprule
{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{AutoFE-Base} & \multicolumn{2}{c}{CAAFE} \\
{} & TabPFN+ & AutoFeat & DFS & GPT-3.5 & GPT-4 \\
\midrule
airlines                   &  \textbf{0.6211} {\tiny $\pm$.04} &           0.6076 {\tiny $\pm$.04} &            0.595 {\tiny $\pm$.04} &            0.619 {\tiny $\pm$.04} &           0.6203 {\tiny $\pm$.04} \\
balance-scale              &           0.8444 {\tiny $\pm$.29} &           0.8438 {\tiny $\pm$.30} &           0.8428 {\tiny $\pm$.31} &            0.844 {\tiny $\pm$.31} &   \textbf{0.882} {\tiny $\pm$.26} \\
breast-w                   &           0.9783 {\tiny $\pm$.02} &           0.9713 {\tiny $\pm$.03} &           0.9783 {\tiny $\pm$.02} &  \textbf{0.9809} {\tiny $\pm$.02} &  \textbf{0.9809} {\tiny $\pm$.02} \\
cmc                        &           0.7375 {\tiny $\pm$.02} &           0.7384 {\tiny $\pm$.02} &           0.7349 {\tiny $\pm$.02} &           0.7383 {\tiny $\pm$.02} &  \textbf{0.7393} {\tiny $\pm$.02} \\
credit-g                   &           0.7824 {\tiny $\pm$.03} &           0.7819 {\tiny $\pm$.03} &           0.7824 {\tiny $\pm$.03} &           0.7824 {\tiny $\pm$.03} &  \textbf{0.7832} {\tiny $\pm$.03} \\
diabetes                   &           0.8427 {\tiny $\pm$.03} &           0.8414 {\tiny $\pm$.03} &           0.8417 {\tiny $\pm$.03} &  \textbf{0.8434} {\tiny $\pm$.03} &           0.8425 {\tiny $\pm$.03} \\
eucalyptus                 &           0.9319 {\tiny $\pm$.01} &  \textbf{0.9321} {\tiny $\pm$.01} &           0.9319 {\tiny $\pm$.01} &           0.9317 {\tiny $\pm$.01} &           0.9319 {\tiny $\pm$.00} \\
jungle_chess..             &           0.9334 {\tiny $\pm$.01} &           0.9197 {\tiny $\pm$.01} &           0.9284 {\tiny $\pm$.01} &           0.9361 {\tiny $\pm$.01} &  \textbf{0.9453} {\tiny $\pm$.01} \\
$\langle Kaggle\rangle$ health-insurance  &           0.5745 {\tiny $\pm$.02} &  \textbf{0.5805} {\tiny $\pm$.03} &           0.5753 {\tiny $\pm$.02} &           0.5745 {\tiny $\pm$.02} &           0.5748 {\tiny $\pm$.02} \\
$\langle Kaggle\rangle$ pharyngitis       &           0.6976 {\tiny $\pm$.03} &           0.6976 {\tiny $\pm$.03} &           0.6976 {\tiny $\pm$.03} &           0.6976 {\tiny $\pm$.03} &  \textbf{0.7078} {\tiny $\pm$.04} \\
$\langle Kaggle\rangle$ kidney-stone      &           0.7883 {\tiny $\pm$.04} &           0.7856 {\tiny $\pm$.04} &  \textbf{0.7929} {\tiny $\pm$.04} &           0.7873 {\tiny $\pm$.04} &           0.7903 {\tiny $\pm$.04} \\
$\langle Kaggle\rangle$ spaceship-titanic &            0.838 {\tiny $\pm$.02} &  \textbf{0.8486} {\tiny $\pm$.02} &           0.8443 {\tiny $\pm$.02} &           0.8383 {\tiny $\pm$.02} &           0.8405 {\tiny $\pm$.02} \\
pc1                        &           0.9035 {\tiny $\pm$.01} &           0.9046 {\tiny $\pm$.01} &           0.9035 {\tiny $\pm$.01} &           0.9087 {\tiny $\pm$.02} &  \textbf{0.9093} {\tiny $\pm$.01} \\
tic-tac-toe                &           0.6989 {\tiny $\pm$.08} &           0.6989 {\tiny $\pm$.08} &           0.6291 {\tiny $\pm$.10} &           0.6989 {\tiny $\pm$.08} &  \textbf{0.9536} {\tiny $\pm$.06} \\
Mean ROC                   &            0.798 {\tiny $\pm$.05} &           0.7966 {\tiny $\pm$.05} &           0.7913 {\tiny $\pm$.05} &           0.7987 {\tiny $\pm$.05} &  \textbf{0.8215} {\tiny $\pm$.04} \\
Mean Rank                  &                              2.75 &                              2.61 &                              2.36 &                              2.96 &                     \textbf{4.32} \\
\bottomrule
\end{tabular}


==> figures/results_table.tex <==
\begin{tabular}{rrrrrr}
\toprule
         &             & \multicolumn{3}{l}{v2} \\
logistic & transformer &      xgb & logistic & transformer &      xgb \\
\midrule
0.766151 &    0.797654 & 0.768980 & 0.779700 &    0.814485 & 0.792080 \\
0.819694 &    0.853341 & 0.821579 & 0.836228 &    0.874529 & 0.840359 \\
\bottomrule
\end{tabular}


==> figures/results_table_means_ranks.tex <==
\begin{tabular}{ll|ll|ll|ll}
\toprule
{} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{AutoFE-Base} & \multicolumn{2}{c}{CAAFE} & \multicolumn{2}{c}{AutoFE-Base + CAAFE} \\
{} &  & AutoFeat & DFS & GPT-3.5 & GPT-4 & GPT-4 + AF & GPT-4 + DFS \\
\midrule
Log. Reg.      &  5.11 &     4.21 &  3.36 &  4.79 &           4.31 &           3.52 &  \textbf{2.69} \\
Random Forest &  4.44 &     4.41 &  4.14 &  4.38 &           4.28 &  \textbf{3.15} &           3.21 \\
TabPFN   &  4.39 &      4.4 &  4.76 &  4.26 &  \textbf{3.06} &           3.27 &           3.86 \\
\bottomrule
\end{tabular}

==> figures/strategies_table_2.tex <==
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single, caption={Simple combination: Example from the Kaggle Kidney Stone dataset.},captionpos=b]
# ('calc_to_urea_ratio', 'Usefulness: The ratio of calcium concentration to urea concentration may be a useful indicator for predicting the formation of calcium oxalate crystals.', 
# Input samples: 'urea': [126.0, 325.0, 282.0], 'calc': [1.16, 7.64, 3.46]
df['calc_to_urea_ratio'] = df['calc'] / df['urea']\end{lstlisting}

        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single, caption={Binning: Example from the Kaggle Spaceship Titanic dataset.},captionpos=b]
# Feature: AgeGroup (categorizes passengers into age groups)
# Usefulness: Different age groups might have different likelihoods of being transported.
# Input samples: 'Age': [30.0, 0.0, 37.0]
bins = [0, 12, 18, 35, 60, 100]
labels = ['Child', 'Teen', 'YoungAdult', 'Adult', 'Senior']
df['AgeGroup'] = pd.cut(df['Age'], bins=bins, labels=labels)
df['AgeGroup'] = df['AgeGroup'].astype('category')\end{lstlisting}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single, caption={String transformation: Example from the Kaggle Spaceship Titanic dataset.},captionpos=b]
# Feature: Deck
# Usefulness: The deck information can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['Deck'] = df['Cabin'].apply(lambda x: x[0] if isinstance(x, str) else 'Unknown')

# Feature: CabinSide
# Usefulness: The side of the cabin can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['CabinSide'] = df['Cabin'].apply(lambda x: x.split('/')[-1] if isinstance(x, str) else 'Unknown')\end{lstlisting}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single, caption={Removing features: Example from the Balance Scale dataset.},captionpos=b]
# Drop original columns
# Explanation: The original columns 'left-weight', 'left-distance', 'right-weight', and 'right-distance' can be dropped as the newly created columns 'left_moment', 'right_moment', and 'moment_difference' capture the relevant information for predicting the 'class'.
df.drop(columns=['left-weight', 'left-distance', 'right-weight', 'right-distance'], inplace=True)
# No more additional columns needed\end{lstlisting}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single, caption={Error Recovery: Example from the Kaggle Health Insurance dataset. The code execution failed because missing values were not considered in the dataframe. In the next iteration code is suggested that can handle missing values.},captionpos=b]
# Feature: Age_difference
# Usefulness: Age difference between upper and lower age can be useful in determining the likelihood of a person applying for a policy.
# Input samples: 'Upper_Age': ['C33', 'C2', 'C3'], 'Lower_Age': ['Owned', 'Rented', 'Rented']
df['Age_difference'] = df['Upper_Age'].str.extract('(\d+)').astype(int) - df['Lower_Age'].str.extract('(\d+)').astype(int)

Feedback: failed with error: cannot convert float NaN to integer. 

# Feature: Age_difference
# Usefulness: Age difference between upper and lower age can be useful in determining the likelihood of a person applying for a policy.
# Input samples: 'Upper_Age': ['C33', 'C2', 'C3'], 'Lower_Age': ['Owned', 'Rented', 'Rented']
df['Age_difference'] = df['Upper_Age'].str.extract('(\d+)').astype(float).fillna(0) - df['Lower_Age'].str.extract('(\d+)').astype(float).fillna(0)\end{lstlisting}

==> figures/valid_datasets_table.tex <==
\begin{tabular}{@{\hskip 0mm}l@{\hskip 0mm}rrrrrrr}
\toprule
 Name & \#Feat. &  \#Cat. &  \#Inst. &  \#Class. &  \#NaNs &  Minor. Class Size & OpenML ID \\
\midrule
 breast-cancer & 10 & 10 & 286 & 2 & 9 & 85 & 13 \\
 dermatology & 35 & 34 & 366 & 6 & 8 & 20 & 35 \\
 haberman & 4 & 2 & 306 & 2 & 0 & 81 & 43 \\
 tae & 6 & 3 & 151 & 3 & 0 & 49 & 48 \\
\bottomrule
\end{tabular}

==> tests/loops.tex <==
%\documentclass{article}
%\usepackage{booktabs}
%\usepackage{listings}
%\usepackage{caption}

%\begin{document}

\begin{table}[h]
    \centering
    \caption{Example code for different strategies}
    \begin{tabular}{lll}
        \toprule
        Strategy & Description & Code \\
        \midrule
        Feature Generation & A feature generated in the & \begin{minipage}[t]{0.6\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\small, frame=single]
df['calc_to_urea_ratio'] = df['calc'] / df['urea']
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        & Kaggle Kidney Stone & \\
        & dataset where a division & \\
        & of two specific features & \\
        & generates a meaningful & \\
        & combination. & \\
        \addlinespace
        Feature Extraction & Three generated features and & \begin{minipage}[t]{0.6\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\small, frame=single]
df['CabinSide'] = df['Cabin'].apply(lambda x: x.split('/')[-1] if isinstance(x, str) else 'Unknown')
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        & explanations for the cmc & \\
        & dataset. The generated & \\
        & features do not improve & \\
        & performance in our & \\
        & evaluations. & \\
        \bottomrule
    \end{tabular}
\end{table}

%\end{document}


==> tests/old_strategies.tex <==
\subsubsection{Strategies}
\label{sec:results:qualitative:strategies}
\paragraph{Simple Combinations} One strategy observed is the combination of the values of two or more features in a simple way. This strategy adds semantic knowledge by combining meaningful features and not others.


\begin{table}[h]
    \centering
    \caption{Example code for different strategies}
    \begin{tabular}{lll}
        \toprule
        Description & Code \\
        \midrule
        \begin{minipage}[t]{0.3\textwidth}
         \textbf{Simple combination:} One strategy observed is the combination of the values of two or more features in a simple way. This strategy adds semantic knowledge by combining meaningful features and not others. Example from the Kaggle Kidney Stone dataset.
        \end{minipage}
        &
        \begin{minipage}[t]{0.7\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single]
# ('calc_to_urea_ratio', 'Usefulness: The ratio of calcium concentration to urea concentration may be a useful indicator for predicting the formation of calcium oxalate crystals.', 
# Input samples: 'urea': [126.0, 325.0, 282.0], 'calc': [1.16, 7.64, 3.46]
df['calc_to_urea_ratio'] = df['calc'] / df['urea']
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        \addlinespace
        \addlinespace
        \addlinespace
        \begin{minipage}[t]{0.3\textwidth}
        \textbf{Binning:} A feature generated in the Kaggle Spaceship Titanic dataset.
        \end{minipage}
        &
        \begin{minipage}[t]{0.7\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single]
# Feature: AgeGroup (categorizes passengers into age groups)
# Usefulness: Different age groups might have different likelihoods of being transported.
# Input samples: 'Age': [30.0, 0.0, 37.0]
bins = [0, 12, 18, 35, 60, 100]
labels = ['Child', 'Teen', 'YoungAdult', 'Adult', 'Senior']
df['AgeGroup'] = pd.cut(df['Age'], bins=bins, labels=labels)
df['AgeGroup'] = df['AgeGroup'].astype('category')
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        \addlinespace
        \addlinespace
        \addlinespace
        \begin{minipage}[t]{0.3\textwidth}
        \textbf{String transformation:} Three generated features and explanations for the cmc dataset. The generated features do not improve performance in our evaluations.
        \end{minipage}
        &
        \begin{minipage}[t]{0.7\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single]
# Feature: Deck
# Usefulness: The deck information can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['Deck'] = df['Cabin'].apply(lambda x: x[0] if isinstance(x, str) else 'Unknown')

# Feature: CabinSide
# Usefulness: The side of the cabin can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['CabinSide'] = df['Cabin'].apply(lambda x: x.split('/')[-1] if isinstance(x, str) else 'Unknown')
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        \addlinespace
        \addlinespace
        \addlinespace
        \begin{minipage}[t]{0.3\textwidth}
        \textbf{Removing features:}
        \end{minipage}
        &
        \begin{minipage}[t]{0.7\textwidth}
        \vspace{-2mm}
        \begin{lstlisting}[language=Python, basicstyle=\scriptsize, frame=single]
[Feature engineering using original columns]

# Drop original columns
# Explanation: The original columns 'left-weight', 'left-distance', 'right-weight', and 'right-distance' can be dropped as the newly created columns 'left_moment', 'right_moment', and 'moment_difference' capture the relevant information for predicting the 'class'.
df.drop(columns=['left-weight', 'left-distance', 'right-weight', 'right-distance'], inplace=True)
# No more additional columns needed
        \end{lstlisting}
        \vspace{-2mm}
        \end{minipage} \\
        \bottomrule
    \end{tabular}
\end{table}


\begin{figure}[h]
    \centering
    \begin{minipage}{\textwidth}
        \begin{lstlisting}[language=Python]
# ('calc_to_urea_ratio', 'Usefulness: The ratio of calcium concentration to urea concentration may be a useful indicator for predicting the formation of calcium oxalate crystals.', 
# Input samples: 'urea': [126.0, 325.0, 282.0], 'calc': [1.16, 7.64, 3.46]
df['calc_to_urea_ratio'] = df['calc'] / df['urea']
        \end{lstlisting}
    \end{minipage}
    \caption{A feature generated in the Kaggle Kidney Stone dataset where a division of two specific features generates a meaningful combination.}
    \label{fig:llm_prompt}
\end{figure}

\paragraph{Binning} Some generated features discretize the observed values into groups. This is a common strategy for feature engineering, where the user has domain-knowledge on the significant inflection points in the feature. Consider a feature such as age, where an age over 18 often has a significantly different meaning.

\begin{figure}[H]
    \centering
    \begin{minipage}{\textwidth}
        \begin{lstlisting}[language=Python]
# Feature: AgeGroup (categorizes passengers into age groups)
# Usefulness: Different age groups might have different likelihoods of being transported.
# Input samples: 'Age': [30.0, 0.0, 37.0]
bins = [0, 12, 18, 35, 60, 100]
labels = ['Child', 'Teen', 'YoungAdult', 'Adult', 'Senior']
df['AgeGroup'] = pd.cut(df['Age'], bins=bins, labels=labels)
df['AgeGroup'] = df['AgeGroup'].astype('category')
        \end{lstlisting}
    \end{minipage}
    \caption{A feature generated in the Kaggle Spaceship Titanic dataset.}
    \label{fig:llm_prompt}
\end{figure}


\paragraph{String transformation} 
For the Spaceship titanic dataset more complex operations on the strings are possible. We show some examples of such string features.
\begin{figure}[H]
    \centering
    \begin{minipage}{\textwidth}
        \begin{lstlisting}[language=Python]
# Feature: Deck
# Usefulness: The deck information can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['Deck'] = df['Cabin'].apply(lambda x: x[0] if isinstance(x, str) else 'Unknown')

# Feature: CabinSide
# Usefulness: The side of the cabin can help identify patterns in the location of cabins associated with transported passengers.
# Input samples: 'Cabin': ['F/356/S', 'G/86/P', 'C/37/P']
df['CabinSide'] = df['Cabin'].apply(lambda x: x.split('/')[-1] if isinstance(x, str) else 'Unknown')
        \end{lstlisting}
    \end{minipage}
    \caption{Three generated features and explanations for the cmc dataset. The generated features do not improve performance in our evaluations.}
    \label{fig:llm_prompt}
\end{figure}

\paragraph{Removing features} 

\begin{figure}[h]
    \centering
    \begin{minipage}{\textwidth}
        \begin{lstlisting}[language=Python]
[Feature engineering using original columns]

# Drop original columns
# Explanation: The original columns 'left-weight', 'left-distance', 'right-weight', and 'right-distance' can be dropped as the newly created columns 'left_moment', 'right_moment', and 'moment_difference' capture the relevant information for predicting the 'class'.
df.drop(columns=['left-weight', 'left-distance', 'right-weight', 'right-distance'], inplace=True)
# No more additional columns needed
        \end{lstlisting}
    \end{minipage}
    \caption{\methodname{} also drops unnecessary features}
    \label{fig:llm_prompt}
\end{figure}

\paragraph{Recovering from errors} 
% TODO: Add reference from method to this
By providing feedback when code execution fails for some features. \methodname{} recovers from these errors within one or two iterations.
\begin{figure}[H]
    \centering
    \begin{minipage}{\textwidth}
        \begin{lstlisting}[language=Python]
# Feature: Age_difference
# Usefulness: Age difference between upper and lower age can be useful in determining the likelihood of a person applying for a policy.
# Input samples: 'Upper_Age': ['C33', 'C2', 'C3'], 'Lower_Age': ['Owned', 'Rented', 'Rented']
df['Age_difference'] = df['Upper_Age'].str.extract('(\d+)').astype(int) - df['Lower_Age'].str.extract('(\d+)').astype(int)

Feedback: failed with error: cannot convert float NaN to integer. 

# Feature: Age_difference
# Usefulness: Age difference between upper and lower age can be useful in determining the likelihood of a person applying for a policy.
# Input samples: 'Upper_Age': ['C33', 'C2', 'C3'], 'Lower_Age': ['Owned', 'Rented', 'Rented']
df['Age_difference'] = df['Upper_Age'].str.extract('(\d+)').astype(float).fillna(0) - df['Lower_Age'].str.extract('(\d+)').astype(float).fillna(0)
        \end{lstlisting}
    \end{minipage}
    \caption{The code execution failed because NaN values were not considered in the dataframe. A new version is suggested that works with NaN values.}
    \label{fig:llm_prompt}
\end{figure}

==> tests/related_work_section_notes.tex <==
%Neural Architecture Search (NAS)-based techniques have also been suggested for automatic feature engineering, including NFS \cite{chen2019neural}, DARTS \citep{liu2018darts}, and NAO \citep{luo2018neural}. However, these approaches may face high computational overhead and difficulties in creating complex features. 
%Various strategies for automatic feature engineering have been investigated in previous studies. Deep Feature Synthesis (DFS) \cite{kanter2015deep} integrates multiple tables for feature engineering by enumerating all potential transformations on features and conducting feature selection based on model performance. In this approach, users need to define the relationships and appropriate column combinations explicitly. Nonetheless, DFS often encounters computational bottlenecks due to the extensive overhead of feature evaluation. To circumvent the need to explore the entire feature space, Cognito \citep{khurana2016cognito} proposes a tree-like exploration of feature space, incorporating handcrafted heuristics traversal strategies, such as breadth-first search and depth-first search. AutoFeat \citep{horn2019autofeat} employs an iterative subsampling of features using beam search.

%Learning-based methods, including LFE \cite{nargesian2017learning} and TransGraph \cite{khurana2018feature}, utilize machine learning models to recommend beneficial transformations. Neural Architecture Search (NAS)-based techniques have also been suggested for automatic feature engineering. For example, NFS \cite{chen2019neural} uses RNN-based controllers to generate transformation sequences for each raw feature. However, these approaches may face high computational overhead and difficulties in creating complex features. To enhance the computational efficiency of NAS, differentiable methods have been introduced. DARTS \cite{liu2018darts} converts the categorical choice into a softmax over all potential operations, resulting in a differentiable learning objective. NAO \cite{luo2018neural} translates the discrete architecture space into a continuous hidden space and optimizes existing architectures in this continuous space. DIFER introduces AutoFE in a continuous vector space and employs a differentiable method to minimize computational complexity, while reinforcement learning-based strategies have been examined by as well \citep{Khurana2017feature, zhang2019automatic}. 

%DIFER: Differentiable Automated Feature Engineering
%The autofeat Python Library for Automated Feature Engineering and Selection

Despite these advancements, none of the existing methods can harness semantic information in an automated manner. Since the possible space of features to evaluate is huge we propose to use this semantic information to reduce computational efficiency and mitigate multiple-testing issues in feature selection.

%Feature engineering is the process of transforming the feature space in a given learning problem to enhance the performance of a trained model. In a typical supervised learning task, the problem can be framed as finding a function F: X → Y using training examples, where F(x) = arg max y S(x, y), X is the input space, Y is the output space, and S: X×Y → R is a scoring function. The objective of automatic feature engineering is to learn a feature representation X → Z that constructs a new feature representation z from the original feature x, ultimately improving the performance of subsequent machine learning tools as much as possible. 

%Not necessary when lots of data is available and deep learning methods used. (expand on this)

%Feature engineering is a central task in data preparation for machine learning. It is the practice of constructing suitable features from given features that lead to improved predictive performance. Feature engineering involves the application of transformation functions such as arithmetic and aggregate operators on given features to generate new ones. Transformations help scale a feature or convert a non-linear relation between a feature and a target class into a linear relation, which is easier to learn. Feature engineering is usually conducted by a data scientist relying on her domain expertise and iterative trial and error and model evaluation.

%Typical engineered features
%The following list[4] provides some typical ways to engineer useful features:

%Numerical transformations (like taking fractions or scaling)
%Category encoder like one-hot or target encoder (for categorical data)[5]
%Clustering
%Group aggregated values
%Principal component analysis (for numerical data)
%Feature construction : building new "physical", knowledge-based parameters relevant to the problem.[6] For example, in physics, construction of dimensionless numbers such as Reynolds number in fluid dynamics, Nusselt number in heat transfer, Archimedes number in sedimentation, construction of first approximations of the solution such as analytical strength of materials solutions in mechanics, etc.[7]

%\subsection{Related work}
%To perform automated feature engineering, some existing approaches adopt guidedsearch in feature space using heuristic feature quality measures (such as information gain) and other surrogate measures of performance [Markovitch and Rosenstein, 2002; Fan et al., 2010]. Others perform greedy feature construction and selection based on model evaluation [Dor and Reich, 2012; Khurana et al., 2016]. Kanter et al. proposed the Data Science Machine (DSM) which considers feature engineering problem as feature selection on the space of novel features. DSM relies on exhaustively enumerating all possible features that can be constructed from a dataset, given sequences generated from a set of transformations, then performing feature selection on the augmented dataset [Kanter and Veeramachaneni, 2015]. Evaluation-based and exhaustive feature enumeration and selection approaches result in high time and memory cost and may lead to overfitting due to brute-force generation of features. Moreover, although deep neural networks (DNN) allow for useful meta-features to be learned automatically [Bengio et al., 2013], the learned features are not always interpretable and DNNs are not effective learners in various application domains. Existing AutoFE approaches can be divided into three categories. Heuristic Approaches: Deep Feature Synthesis (DFS), the component of Data Science Machine (Kanter and Veeramachaneni, 2015), rst enumerates all transformations on all features and then performs feature selection directly based on the improvement of model performance. One Button Machine (Lam et al., 2017) adopts a similar approach. However, this expansion-reduction approach suers from a severe computational performance bottleneck due to the huge feature evaluation overhead. To avoid enumerating the entire feature space, Cognito (Khurana et al., 2016) introduces a tree-like exploration of feature space and presents handcrafted heuristics traversal strategies such as breadth-rst search and depth-rst search. AutoFeat (Horn et al., 2019) iteratively subsamples features using beam search. However, heuristic approaches cannot learn from past experiences and thus has a low search eciency. Learning-Based Approaches: To explore feature space eciently, learning-based AutoFE methods have been proposed. LFE (Nargesian et al., 2017) trains an MLP and recommends the most likely useful transformation for each raw feature. However, it does not support transformation composition and works only for classication tasks. TransGraph (Khurana et al., 2018) trains a Q-learning agent to decide which transformation should be applied. Due to performing each transformation on all features, TransGraph suers from feature explosion and low computational eciency. NAS-Based Approaches: Neural Architecture Search (Elsken et al., 2019) has aroused signicant research interests in the eld of AutoML (He et al., 2020). The reinforcement learning-based NAS method (Zoph and Le, 2017) views the structure of a neural network as a variable-length string. Then, it uses a recurrent network as the controller to generate such strings and trains the controller with policy gradient. This approach can be adopted into AutoFE. For instance, NFS (Chen et al., 2019), the current SOTA AutoFE method, utilizes several RNN-based controllers to generate transformation sequences for each raw feature. However, evaluating enormous sequences results 2 in substantial computational overhead. Most importantly, due to the side eects of reducing binary transformations to unary ones, NFS cannot generate complex features like. To improve the computational eciency of NAS, dierentiable methods have been proposed. DARTS (Liu et al., 2018) relaxes the categorical choice to a softmax over all possible operations, leading to a dierentiable learning objective. NAO (Luo et al., 2018) maps the discrete architecture space to a continuous hidden space and optimizes existing architectures in the continuous spac Numerous studies have been conducted on automatic feature engineering. Reinforcement learning-based strategies have been explored by Khurana et al. (2018) [17] and Zhang et al. (2019) [19]. These methods, however, necessitate multiple rounds of attempts, where new feature sets are generated and evaluated in each round, rendering them impractical for industrial tasks. Transfer learning or meta-learning-based strategies have also been proposed for automatic feature engineering [20], [21]. Notable works in this area include "Deep feature synthesis: Towards automating data science endeavors" [22], which developed the Data Science Machine to derive predictive models from raw data automatically, and "SAFE: Scalable Automatic Feature Engineering Framework for Industrial Tasks" [23], which proposed a staged method named SAFE, providing efficiency, scalability, interpretability, and promising performance. Another related work is "Cognito: Automated Feature Engineering for Supervised Learning" [24], a system that performs automatic feature engineering for supervised learning by exploring feature construction choices in a hierarchical and non-exhaustive manner while maximizing model accuracy through a greedy exploration strategy. To the best of our knowledge none of these methods use semantic information.


==> tests/test.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\begin{figure}[H]
\centering
\begin{minipage}{\textwidth}
\begin{lstlisting}[caption={User-provided dataset description: Tic-Tac-Toe Endgame database},label=block1]
This database encodes the complete set of possible board configurations at the end of tic-tac-toe games, where "x" is assumed to have played first. The target concept is "win for x" (i.e., true when "x" has one of 8 possible ways to create a "three-in-a-row").
\end{lstlisting}
\begin{lstlisting}[caption={LLM-generated iteration 1},label=block2]
Iteration 1
\end{lstlisting}
\begin{lstlisting}[language=Python, caption={LLM-generated code for adding features},label=block3]

('number-of-x-wins', 'Number of ways x can win on the board')
Usefulness: Knowing the number of ways x can win on the board can be useful in predicting whether x has won the game or not.
Input samples: 'top-left-square': [2, 2, 1], 'top-middle-square': [1, 2, 0], ...
df['number-of-x-wins'] = ((df['top-left-square']==1) & (df['top-middle-square']==1) & (df['top-right-square']==1)).astype(int) + ((df['middle-left-square']==1) & (df['middle-middle-square']==1) & (df['middle-right-square']==1)).astype(int) [...]
\end{lstlisting}
\begin{lstlisting}[caption={Feedback from executed algorithm},label=block4]
Performance before adding features ROC 0.888, ACC 0.700.
Performance after adding features ROC 0.987, ACC 0.980.
Improvement ROC 0.099, ACC 0.280. The code was executed and changes to df were retained.
\end{lstlisting}
\end{minipage}
\caption{Exemplary run of \methodname{} on the Tic-Tac-Toe Endgame database.}
\label{fig:llm_prompt}
\end{figure}

\end{tikzpicture}

